MOVE: Unsupervised Movable Object Segmentation and Detection

We introduce MOVE, a novel method to segment objects without any form of supervision. MOVE exploits the fact that foreground objects can be shifted locally relative to their initial position and result in realistic (undistorted) new images. This property allows us to train a segmentation model on a dataset of images without annotation and to achieve state of the art (SotA) performance on several evaluation datasets for unsupervised salient object detection and segmentation. In unsupervised single object discovery, MOVE gives an average CorLoc improvement of 7.2% over the SotA, and in unsupervised class-agnostic object detection it gives a relative AP improvement of 53% on average. Our approach is built on top of self-supervised features (e.g. from DINO or MAE), an inpainting network (based on the Masked AutoEncoder) and adversarial training.

==> MOVE - NeurIPS 2022_arXiv_resize2048/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> MOVE - NeurIPS 2022_arXiv_resize2048/tables/os-comp.tex <==

\begin{table*}[!t]
  \centering
  \small
\caption{ {Comparison to the unsupervised saliency detection methods on 3 benchmarks} %
\label{tab:salient-comp}
}
\vspace{1em}
\small
        \begin{tabularx}{\linewidth}{@{}X 
        @{\hspace{.5em}}c@{\hspace{.5em}}c@{\hspace{.5em}}c@{\hspace{.5em}}c@{\hspace{.5em}}c@{\hspace{.5em}}c@{\hspace{.5em}}c@{\hspace{.5em}}c@{\hspace{.5em}}c@{}}
        \toprule
        \multirow{2}{*}{Model}
         &\multicolumn{3}{c}{DUT-OMRON~\cite{yang2013saliency}}
         &\multicolumn{3}{c}{DUTS-TE~\cite{wang2017learningDUTS}}
         &\multicolumn{3}{c}{ECSSD~\cite{shi2015hierarchical}}\\   \cmidrule{2-10}
         &\small Acc &\scriptsize IoU&\scriptsize max$F_\beta$
         &\small Acc &\scriptsize IoU&\scriptsize max$F_\beta$
         &\small Acc &\scriptsize IoU&\scriptsize max$F_\beta$\\
        \midrule
        HS~\cite{yan2013hierarchical}
        &.843&.433&.561
        &.826&.369&.504
        &.847&.508&.673\\
        wCtr~\cite{zhu2014saliency}
        &.838&.416&.541
        &.835&.392&.522
        &.862&.517&.684\\
        WSC~\cite{li2015weighted}
        &.865&.387&.523
        &.862&.384&.528
        &.852&.498&.683\\
        DeepUSPS~\cite{nguyen2019deepusps}
        &.779&.305&.414
        &.773&.305&.425
        &.795&.440&.584\\
        SelfMask pseudo$^{\star}$~\cite{Shin2022selfmask}
        &.811&.403&-
        &.845&.466&-
        &.893&.646&-\\
        BigBiGAN~\cite{voynov2020big}
        &.856&.453&.549
        &.878&.498&.608
        &.899&.672&.782\\
        E-BigBiGAN~\cite{voynov2020big}
        &.860&.464&.563
        &.882&.511&.624
        &.906&.684&.797\\
        Melas-Kyriazi et al.~\cite{melaskyriazi2021finding}
        & .883 & .509 & -
        & .893 & .528 & - 
        &.915 & .713 & -\\
        LOST~\cite{LOST}
        &.797&.410&.473
        &.871&.518&.611
        &.895&.654&.758\\
        Deep Spectral~\cite{melas2022}
        &-&.567&-
        &-&.514&-
        &-&.733&-\\
        TokenCut~\cite{wang2022self}
        &.880&.533&.600
        &.903&.576&.672
        &.918&.712&.803\\
        FreeSOLO~\cite{wang2022freesolo}
        &.909 & .560 & .684
        &.924 & .613 & .750
        &.917 & .703 & .858\\
        \bf \methodname (Ours)
        &\textbf{.923}&\textbf{.615}&\textbf{.712}
        &\textbf{.950}&\textbf{.713}&\textbf{.815}
        &\textbf{.954}&\textbf{.830}&\textbf{.916}\\ %
        \midrule
        LOST~\cite{LOST} + Bilateral 
        &.818&.489&.578
        &.887&.572&.697
        &.916&.723&.837\\
        
        

        TokenCut~\cite{wang2022self} + Bilateral %
        &.897&.618&.697
        &.914&.624&.755
        &.934&.772&.874\\
        

        \bf \methodname (Ours) + Bilateral %
        &\textbf{.931}&\textbf{.636}&\textbf{.734}
        &\textbf{.951}&\textbf{.687}&\textbf{.821}
        &\textbf{.953}&\textbf{.801}&\textbf{.916}\\ %
        \midrule
        SelfMask on pseudo$^{\star}$ ~\cite{Shin2022selfmask}
        &.923&.609&.733
        &.938&.648&.789
        &.943&.779&.894\\ %
        SelfMask on pseudo$^{\star}$ ~\cite{Shin2022selfmask} + Bilateral%
        &\textbf{.939}&\textbf{.677}&\textbf{.774}
        &.949&.694&.819
        &.951&.803&.911\\ %
        \bf SelfMask on \methodname (Ours)
        &.933&.666&.756
        &\textbf{.954}&\textbf{.728}&\textbf{.829}
        &\textbf{.956}&\textbf{.835}&\textbf{.921}\\ %
        \bf SelfMask on \methodname (Ours) + Bilateral 
        &.937&.665&.766
        &.952&.687&.827
        &.952&.800&.917\\ %
        \bottomrule
        \end{tabularx}
        \raggedright
        \footnotesize{
        $^{\star}$We found that SelfMask's $\max F_{\beta}$ metric was computed with an optimal threshold for each image instead of the entire dataset as in other methods; we re-evaluated their model for a fair comparison} 
\end{table*}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
